VACT: A Video Automatic Causal Testing System and a Benchmark

With the rapid advancement of text-conditioned Video Generation Models (VGMs), the quality of generated videos has significantly improved, bringing these models closer to functioning as ``*world simulators*'' and making real-world-level video generation more accessible and cost-effective. However, the generated videos often contain factual inaccuracies and lack understanding of fundamental physical laws. While some previous studies have highlighted this issue in limited domains through manual analysis, a comprehensive solution has not yet been established, primarily due to the absence of a generalized, automated approach for modeling and assessing the causal reasoning of these models across diverse scenarios. To address this gap, we propose VACT: an **automated** framework for modeling, evaluating, and measuring the causal understanding of VGMs in real-world scenarios. By combining causal analysis techniques with a carefully designed large language model assistant, our system can assess the causal behavior of models in various contexts without human annotation, which offers strong generalization and scalability. Additionally, we introduce multi-level causal evaluation metrics to provide a detailed analysis of the causal performance of VGMs. As a demonstration, we use our framework to benchmark several prevailing VGMs, offering insight into their causal reasoning capabilities. Our work lays the foundation for systematically addressing the causal understanding deficiencies in VGMs and contributes to advancing their reliability and real-world applicability.

==> sec/2_mainbody.tex <==

\section{Pipeline of automatic causal rule testing}

\subsection{Scenario-based causal rule testing}

% Our tests are started from some \textbf{scenario}s. A \textbf{scenario} is defined as a short text description of an event, like ``something is thrown into a swimming pool'' in Figure~\ref{fig:bad_case}. Given a scenario, the properties of some objects or events involved can be regarded as variables, and there are causal relationships between these variables. A causal graph and a causal system can be used to model these relationships. Here, we call the functions to define the relationships as \textbf{causal rules}. At the same time, the rules consist of a \textbf{test case}, which is the unit of our tests. As mentioned in the introduction, a scenario may have different causal choices and therefore can correspond to multiple different test cases, if we choose different factors (therefore, different rules). Here, we provide a mathematical definition of the causal graph and causal system.
Our tests begin with \textbf{scenario}s, short text descriptions of an event, such as ``something is thrown into a swimming pool'' (in Figure~\ref{fig:bad_case}). Each scenario involves variables representing object or event properties, linked by causal relationships modeled as a causal graph and a causal system.

\begin{definition}[Causal graph and system~\citep{causality2009pearl}] 
A deterministic \textbf{causal system} over a set of variables $\mathbf{V}$ is a directed acyclic graph $G$ with the node set $\mathbf{V}$ and edge set $\mathbf{E}$, and a series of structural equations $V_j=f_j(pa(V_j))$ for every $V_j\in \mathbf{V}$, where $pa(V_j)=\{V_k\in \mathbf{V}:V_k\to V_j\in \mathbf{E}\}$ are the parents of the node $V_j$. The graph $G$ is called the \textbf{causal graph}. Furthermore, let $\mathbf{X}=\{V_j\in\mathbf{V}: pa(V_j)=\emptyset\}$ be the \textbf{root} (\textbf{cause}) variables and $\mathbf{Y}=\mathbf{V} \setminus \mathbf{X}$ be the \textbf{non-root} (\textbf{outcome}) variables.

\end{definition}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/causal_graph_pool.pdf}

    \caption{An example causal graph and system: ``\textit{throwing something into a swimming pool}''. \textcolor{cyan}{Blue} denotes root nodes and \textcolor{orange}{orange} denotes non-root nodes. Physical explanation can be found in~\citep{dropimpact} Figure 6.}
    \label{fig:causal_graph_pool}
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{figs/pipeline of vact_v3.pdf}
    
    \caption{Pipeline of VACT. The pipeline mainly consists of four parts: causal system (\ie test case) proposal (\textcolor{Goldenrod}{yellow}), text prompt generation, (\textcolor{LimeGreen}{green}), video generation (\textcolor{Cyan}{blue}), answer retrieval and evaluation (\textcolor{pink}{pink}). The pipeline receive a sentence describe a scenario as input and automatically evaluate video generation models \textit{without} any human supervision or annotation.}
    
    \label{fig:pipeline}
\end{figure*}

We illustrate this with an example in Figure~\ref{fig:causal_graph_pool}, where the system captures commonsense physical knowledge—for instance, density determines whether an object will sink, while speed, size, and density collectively influence the splash.
The directed edges in the graph represent causal relationships between variables, such as the edge ``high density'' $\to$ ``object sink'' indicating causation, while there is no causal effect between ``large size'' and ``object sink'', since a dense object will sink regardless of its size.
Root variables (\textcolor{cyan}{blue}) are basic conditions of a scenario that can be directly manipulated. Non-root variables (\textcolor{orange}{orange}) are outcomes of other variables that cannot be directly adjusted but may influence other factors. For example, the non-root variable ``splash'' causes ``ripples'', which in turn causes ``sparkling''~\citep{dropimpact}.
The basic unit of our VACT is a causal system, consisting of these rules (\ie the equations). One scenario may generate different test cases depending on the selected factors.
%and $\mathbf{Y}=\mathbf{V} \setminus \mathbf{X}$. Then $\mathbf{X}$ is called the set of root (or cause) variables, and $\mathbf{Y}$ is called the set of non-root (or outcome) variables. 
%From the definition we can conclude that $\mathbf{Y}=f(\mathbf{X})$ for some function $f$. We call $f$ the \textbf{rule} in this scenario.

% In this article, for the sake of clarity, we require all variables to take Boolean values. Therefore, a causal system is a series of Boolean functions. These Boolean functions are a reasonable simplification of various physical relationships in nature. For those physical properties that take continuous values, we can actually avoid complex calculations and highlight the ``essence'' of their causal relationships by binarizing them --- for example, simplifying the continuous value of speed to ``fast'' and ``slow'', and simplifying the mass of an object to ``light'' and ``heavy''. In fact, this simplification is also in line with human commonsense, because in daily life we generally use these binary rather than continuous values to make commonsense judgments and think.

For the sake of clarity, all variables in our system are \textit{Boolean}, meaning the rules are Boolean functions. This simplification reasonably abstracts physical relationships, avoiding complex calculations while preserving essential causal structures. Continuous properties, such as speed or mass, can be binarized (\eg ``fast'' \vs ``slow'' or ``light'' \vs ``heavy''), as we often make judgments using such discrete categories in daily life. Additionally, the variables must be visually discernible\footnote{The visualization here is a relative requirement. For example, although the density is essentially invisible, we can infer the density of an object through its visible material.} (\textit{visibility}) to ensure suitability for video evaluation, and all root nodes can be set \textit{independently}.
%
% We define a 
% For each specific scenario, let $\mathbf{X}=(X_1,X_2,\dots,X_{m_1})$ be all root (cause) variables, and let $\mathbf{Y}=(Y_1,Y_2,\dots,Y_{m_2})$ be all non-root (outcome) variables. All variables are binary. Let $G$ be a directed acyclic graph (DAG) with node set $\mathbf{V}=\{X_1,X_2,\dots,X_{m_1},Y_1,Y_2,\dots,Y_{m_2}\}.$ There is no parent for the cause variables but each outcome variable $Y_i$ has some parents, denoted by $pa(Y_i).$ We assume that the value of $Y_i$ is determined by its parents, that is, $Y_i=f_i(pa(Y_i)),$ where $f_i$ is called the rule of $Y_i.$ It can also be equivalently represented as $\mathbf{Y}=f(\mathbf{X}).$
%
%Figure~\ref{fig:causal_graph_pool} provides a possible causal graph and system about the scenario in Figure~\ref{fig:bad_case} ``\textit{throwing something into a swimming pool}''. The nodes represent some main variables in the scenario. The links and the rules (Boolean functions) explain the causal relations. For example, the system describes some physics commonsense that density affects whether the object will sink and speed, size and density affect the splash.
%
%For example, consider the scenario in Figure~\ref{fig:bad_case}: ``\textit{throwing something into a swimming pool}'', a possible causal graph and system are shown in Figure~\ref{fig:causal_graph_pool}. The nodes represents some main variables in this scenario, including the object properties like dense and size, the throwing speed, which can make a difference in some obvious and important results, such as whether there is splash and ripples, and whether objects sink into the water. In the figure, we label the ``root'' factors as blue and ``non-root'' factors as orange, where the ``root'' factrs are considered as the cause of other factors but the ``non-root'' factors, in addition to being results of other factors, can also be the cause. For example, the ``splash'' is the cause of the ``sparkling'' because sparkling is caused by the instability of the water surface.
If a video generation model learns the physical laws of a scenario, it should have learned the rule $f$. Thus, by analyzing variable states in generated videos under different conditions, we can assess whether the model understands the underlying law.

\subsection{LLM-aided automatic generation of test cases}
\label{subsec:auto_label}

As discussed in Section~\ref{sec:intro}, extracting key causal rules from scenarios is challenging due to their inherent complexity and diversity. This task requires both creativity (to imagine alternative scenarios) and commonsense reasoning (to recognize common causal patterns). Fortunately, the advanced commonsense reasoning capabilities of Large Language Models (LLMs) enable automation of this process. We designed a multi-step annotation method that leverages LLMs, incorporating task splitting, rule checking, and self-correction to ensure accuracy and reliability.

As illustrated in Figure~\ref{fig:pipeline} (\textcolor{Goldenrod}{yellow} part), our system accepts a scenario (a brief textual description) and prompts the LLM to sequentially perform the following steps: 1) identify key causal factors and outcomes within the scenario, 2) discover relationships between these elements to construct a causal graph, and 3) derive Boolean expressions representing the discovered relationships.

After each step, we implement self-checking and rule-checking mechanisms. If errors are identified, such as formatting issues, unusual relationships, isolated nodes in the causal graph, or mismatched Boolean expressions, we provide explicit error feedback to the LLM, prompting it to self-correct. If no errors are found, the model is prompted to perform an additional self-check. The step-splitting and self-correction strategy ensure that errors are detected and corrected, significantly improving the overall quality of generated outputs. The final test case comprises both the Boolean expression and the original scenario text. Detailed generation requirements, inspection indicators, and a comprehensive description of the process can be found in Appendix~\ref{app:automatic_generation_detail}.

% As discussed in Section~\ref{sec:intro}, extracting key causal rules from a scenario is challenging due to complexity and diversity, requiring creativity (imagining alternative scenarios) and commonsense (identifying common causal patterns). Fortunately, the advanced commonsense reasoning ability of LLMs enables automation of this task. We designed a multi-step annotation process using LLMs with task splitting, rule checking, and self-correction.
% As shown in Figure~\ref{fig:pipeline} (\textcolor{Goldenrod}{yellow} part), the system takes a scenario (a short text description) as input and prompts the LLM to: 1) analyze key causal factors and results in the scenario, 2) discover the relationships between them to construct a causal graph linking variables, and 3) derive Boolean expressions representing these relationships. These three steps are carried out sequentially.
% We also adopt self-check and/or rule-check after each step. If any error has been found in the previous generation, we provide the error information to the LLM and prompt LLM to fix it leveraging the LLM's self-correction ability to improve result reliability. Otherwise, we prompt LLM to operate self-check. These errors could be the output format, uncommon relationships found, isolated nodes in the causal graph, or Boolean expressions that do not match the causal graph, \etc. These check make sure errors that occur at each step can be fixed as early as possible. 
% Although the intermediate generations are all included in the final causal system, we found that this multi-step design significantly improves the generation quality of the model.
% The final test case consists of the expression with the scenario text.
%As we discussed in section~\ref{sec:intro}, extracting the important causal rules in a given scenario is not trivial due to the complexity and diversity. This process is creative because it requires imagining other possible scenarios from one scenario, and retaining common and main possibilities while removing overly corner-case scenarios, which relies heavily on human commonsense, intuition, and inspiration. Fortunately, current high level of commonsense understanding of LLMs make it possible to complete this task with the aid of LLMs. We designed a multi-step automatic annotation process using LLMs with task splitting, rule checking and self-correction. As shown in Figure~\ref{fig:pipeline} (\textcolor{Goldenrod}{yellow} part), the system receives a scenario (i.e., a short text description) as input, and we prompt LLM to perform the following three steps in steps: 1) Analyze the main factors that may cause obvious results in the current scenario 2) Based on the above analysis, construct these possible variables and their results into a causal graph to preliminarily establish the causal relationship between them 3) Based on the causal graph, further characterize the Boolean expression of the relationships between these variables. Finally, this Boolean expression (causal system) and the input scenario together constitute a test case.
% For detailed generation requirements, inspection indicators and the full process, see Appendix~\ref{app:automatic_generation_detail}.% The model will start to complete the next task until the maximum number of attempts is reached or the external check and self-check are passed.
%We prompt the LLM to complete these tasks in sequence through multiple rounds of dialogue. During this process, the complete dialogue history is always saved in the context window. For details about our various requirements and inspection indicators for generation and a more detailed generation process, please see the appendix~\ref{app:automatic_generation_detail}.

\paragraph{Crowd experiments} 
We evaluate the effectiveness of the automatic generation by crowd experiments. We collected 20 diverse scenarios (listed in Appendix~\ref{app:scenario_list}) and generated three causal systems for each, 60 in total. For comparison, three undergraduates manually annotated the same scenarios using identical instructions given to the LLM, resulting in another 60 \textit{human-annotated} causal systems. Then, another five undergraduates blindly scored both human and LLM annotations based on three criteria: \textit{requirement} (adherence to visibility, binarity and root independence), \textit{rationality} (reasonableness of factor selection), and \textit{soundness} (accuracy of causal rules). For each criteria, the scores range from 1 which means there are essential error to 4 which means the annotation perfectly meets the requirement.  The average score from 5 scorer and 60 samples are reported in Table~\ref{tab:crowd_average}. LLM-generated annotations surprisingly \textbf{outperformed} those from human, demonstrating the effectiveness of the LLM-driven process and its strong alignment with human reasoning. 
We also provide the details of the crowd experiments, the score distribution of each scorer and further analysis in Appendix~\ref{app:crowd_exp}.

\addtolength{\tabcolsep}{-3pt} 
\begin{table}[htpb]

    \caption{Average scores from crowd experiments}

    \label{tab:crowd_average}
    \centering
    \begin{tabular}{lcccc}
    \toprule
    Source& Requirement & Rationality & Soundness & Average \\ \midrule
    \textbf{LLM}   &  $\textbf{3.91}\mathsmaller{\pm 
 0.02}$ & $\textbf{3.49}\mathsmaller{\pm 0.04}$ & $\textbf{3.78}\mathsmaller{\pm 0.03}$ & $\textbf{3.73}\mathsmaller{\pm 0.02}$\\
    \textbf{Human} &  $3.80\mathsmaller{\pm 0.03}$ & $\textbf{3.51}\mathsmaller{\pm 0.04}$ & $3.63\mathsmaller{\pm 0.04}$ & $3.65\mathsmaller{\pm 0.03}$ \\ \bottomrule
    \end{tabular}
\end{table}


%We operate a crowd experiments to prove the effectiveness of the automatic generation of causal graphs. We collect 20 scenarios and generate three causal systems for each scenario. As comparison, we invited three undergraduates to manually annotate these scenes providing them with the same instructions as for LLM annotation. Then, we invited another five undergraduates to blindly score the annotations from both human and LLM sources; here we distinguished three scoring criteria: requirement (whether the annotation meets requirements like visibility), rationality (whether the choices of factors are rational), soundness (whether the rules are correct). The results are shown in Table~\ref{tab:crowd_average}. We found that LLM annotations have better performance than undergraduate-level human annotations. This proves that the LLM automatic annotation process can effectively complete this complex task and is highly aligned with human tendencies. Please refer to the Appendix~\ref{app:crowd_exp} for details and more analysis on the crowd experiment.

% \begin{wraptable}{r}{5.5cm}
%     \caption{Scores from crowd experiments of human- and LLM-sourced causal system. The $\pm$ shows the standard deviation calculated by bootstrap.}
%     \label{tab:crowd_average}
%     \centering
%     \begin{tabular}{lcccc}
%     \toprule
%     Source& Requirement & Rationality & Soundness & Average \\ \midrule
%     LLM   &  $\textbf{3.91}\mathsmaller{\pm 
%  0.02}$ & $\textbf{3.49}\mathsmaller{\pm 0.04}$ & $\textbf{3.78}\mathsmaller{\pm 0.03}$ & $\textbf{3.73}\mathsmaller{\pm 0.02}$\\
%     Human &  $3.80\mathsmaller{\pm 0.03}$ & $\textbf{3.51}\mathsmaller{\pm 0.04}$ & $3.63\mathsmaller{\pm 0.04}$ & $3.65\mathsmaller{\pm 0.03}$ \\ \bottomrule
%     \end{tabular}
% \end{wraptable}


\subsection{Automatic intervention experiment pipeline}
\label{ssec:automatic}

Given a causal system, our testing as intervention experiments contains five parts: sampling, prompt generation, video generation, answer retrieval, and evaluation, as shown in Figure~\ref{fig:pipeline}. Details and the prompt used in these steps are in Appendix~\ref{app:test_pipeline}.


\textbf{Sampling}.
In our intervention experiments, observations are videos characterized by varying condition values $\mathbf{X}$.
We sample diverse combinations of root values $\mathbf{X}$ for these intervention. The sample size for each $\mathbf{X}$ value combination is determined by metrics discussed in Section~\ref{sec: three levels}. Given the high cost of video generation, it is crucial to minimize the number of videos needed while ensuring accurate and stable metrics measurement. Therefore, we (1) conduct preliminary experiments to determine the minimum number of samples that can ensure the relative stability and validity of each metric and (2) strategically share generated videos across different metrics whenever feasible. Finally, the number of sample for each $\mathbf{X}$ value combination is set to the maximum requirement across the three metrics. We provide the details of samples in Appendix~\ref{app:sample_strategy} and the preliminary experiments used to determine the minimum number in Appendix~\ref{app:sample_size_exp}. Through our experiments, we conduct that approximately 30 to 45 videos per causal system are sufficient to achieve stable evaluations.
%We sample some combinations of root values $\mathbf{X}$ as intervention experiments. The number of samples for each $\mathbf{X}$ value is determined by the metrics we use (in Section~\ref{sec: three levels}) and described in Appendix~\ref{app:sample_strategy}. In our experiments, we took approximately 20 - 40 (\textcolor{red}{need to check}) samples for each causal system. 

%specify the value of root nodes $\mathbf{X}$, that is, we manipulate the state of cause variables in the scenario. The distribution we set for $\mathbf{X}$ is related to the metric we use, described in Section~\ref{sec: three levels}.


\textbf{Prompt generation}. 
Given $\mathbf{X}$ values, we use an LLM to generate sentences to constrain restrict the variables in the scenario as meeting the given values. For example, in the scenario ``throwing something into a swimming pool'', the prompt ``\textit{a large rock was thrown quickly into the pool}'' sets three root variables: high density, large size, and high speed to true, while another prompt ``\textit{a tiny stone is gently placed on the water}'' alert large size and high speed to false. These sentences serve as text prompts for video generation.


%Given the values of $\mathbf{X}$, we can generate a sentence to restrict the variables in the scenario as meeting the given values. For example, for the scenario ``throwing something into the swimming pool'', a prompt like `` \textit{a large rock was thrown quickly into the pool}'' can restrict the values of factors ``\textit{high density}'', ``\textit{large size}'' and ``\textit{high speed}'' as all true; while `\textit{`a tiny stone is gently placed on the water}'' corresponding the ``\textit{large size}'' and ``\textit{high speed}'' as false.
% These sentences are used as text prompts for the generation of videos. %We consider two types of prompts: coarse and detailed. For the coarse prompt, we only specify the value $\mathbf{X} = \mathbf{x}$; for the detailed prompt, we specify both $\mathbf{X} = \mathbf{x}$ and $\mathbf{Y} = f(\mathbf{x})$. The formal one is only used for % In either case, if VGMs have sufficient text understanding and conditioned generation capabilities, they can generate videos that match the given $X$ and corresponding $Y$ values.

\textbf{Video generation}. 
The prompts generated are provided to the tested VGM. These models are treated as black boxes, requiring no constraints on their structure.


\textbf{Answer retrieval}.
Each generated video serves as an observation of the intervention experiments for the causal system. We check (1) whether it follows the text description of variable values $\mathbf{X}$ and (2) whether the generated values $\mathbf{Y}$ align with the causal rules. 
Following \citet{meng2024worldsimulatorcraftingphysical}, we use a vision-LLM (VLLM) to retrieve the observed values $\hat{\mathbf{X}}$ and $\hat{\mathbf{Y}}$ in each video, by prompting the VLLM with the video and some ``\textit{yes-no}'' questions (\ie \textit{probes}). These probes are also generated by an LLM given the variable list of a causal system. Notice that our variable has been required to be binary when generating test cases, so the generation of these questions is a very simple tasks.

%Each video generated is an observation of the intervention experiments about this causal system. To measure the causal understanding of VGMs, we need to know (1) whether they faithfully follow the text's description of the choice of variable values $\mathbf{X}$ and (2) whether they generate values $\mathbf{Y}$ that match the causal rules? Like~\citet{meng2024worldsimulatorcraftingphysical}, we use an multi-modal LLM (VLLM) with video understanding ability to retrieve the value of both $\mathbf{X}$ and $\mathbf{Y}$ in the videos. Specifically, we prompt a generated video with some ``yes-no'' questions (which is generated simultaneously when the graph is generated) to the VLLM and collect the answer as the ``\textit{observed value}'' (denoted by $\hat{\mathbf{X}}$ and $\hat{\mathbf{Y}}$).
% use a large language model that can accept both video and text as input to query the content of the video, thereby obtaining the observed states of the variables in the scenario within the generated video, denoted by $\hat{\mathbf{X}}$ and $\hat{\mathbf{Y}}$.

%\textbf{Evaluation}. For the video generation model, the ideal scenario is when $\mathbf{X} = \hat{\mathbf{X}}$ and $\mathbf{Y} = \hat{\mathbf{Y}}$. However, when they are not equal, it may indicate errors in the generation process or the model's understanding of the objective world. In Section~\ref{sec: three levels}, we will propose several metrics to measure these deviations.
% With the observation, we can evaluate the causal behavior of the tested model. In Section~\ref{sec: three levels}, we will propose several metrics.

We adopt an LLM and a VLLM to automate the steps \textit{prompt generation}, \textit{probe generation} and \textit{Answer retrieval}. To ensure the correctness, we performed random manual checks. We found that the vast majority of the results are reliable. The check results are shown in Appendix~\ref{app:manual_check}. 


\section{Three levels of causal ability and the corresponding metrics}

\label{sec: three levels}
% In the main part of the section, we introcude the scenario-based scores.
To assess the deviation of the model's understanding of the objective world, we propose a three-level framework of causal capabilities with corresponding evaluation metrics. The mathematical definitions are provided in Appendix~\ref{app:detailed_def_for_metrics}. Here, we focus on an intuitive description.

\paragraph{Text consistency}
The first level assesses whether the model accurately reflects the state of every variable described in the prompt. By generating a video from a detailed prompt specifying variable values, the resulting video should correctly reflect those values. It is a fundamental requirement for not only the general usage of video generation models but also our intervention experiments because we need to control video variables through text.
The similar metrics have proposed in some previous benchmarks, such as video-text consistency in VBench~\citep{huang2024vbench}, but it is still different. In our test, a video generation requires multiple important but complex attributes simultaneously, and there are some uncommon combinations. Therefore, our test is more difficult than similar evaluations.

We use two types of prompts: the standard prompts (described in Section~\ref{ssec:automatic} and also used in the next two metrics) specifies \textit{all root} variables $\mathbf{X}$. In addition, we generate prompts constraining all variable values (including roots $\mathbf{X}$ and non-roots $\mathbf{Y}$), describing not only the condition but also expected results in the scenario. These two types correspond to the ``\textit{root}'' score and ``\textit{all}'' score, respectively. 
The first type aligns with common real-world application, where the results are not stated before generating. The second serves as a complementary test about whether explicitly stating expected outcomes helps the model generate correct physical behaviors. For each setting, we measure text consistency using the \textit{average accuracy} of whether the observed values match the described ones.

% The metric $s_1^{\mathrm{root}}\propto \sum_{i,V\in\mathbf{V}}1(X_i=\hat{X}_i)$ measures the accuracy across all variables. Additionally, we also introduce $s_1^{\mathrm{all}}\propto \sum_{i,X\in\mathbf{X}}1(X_i=\hat{X}_i)$, which focuses on the consistency of cause variables. These metrics evaluate whether the model has learned to maintain consistent representations of the input variables, reflecting its ability to adhere to the provided descriptions.


\paragraph{Generation consistency}
The second level evaluates whether the model stably produces the stable and predictable outcomes given identical causes $\mathbf{X}$, or if its outcomes vary arbitrarily due to unrelated factors like random seed or wording differences.
%The second level evaluates whether the model consistently produces the same outcomes given identical causes $\mathbf{X}$. This indicates whether the model has internalized stable input-output rules, or if its outcomes vary arbitrarily due to unrelated factors like random seed or wording differences.
To measure this, we group the samples by identical $\mathbf{X}$ values, and calculate the mean variance of outcomes $Y_j$ within each group. Since grouping is based on $\mathbf{X}$, errors arise if text consistency (level one) is imperfect. To address this, we use two scoring criteria: ``\textit{truth}'' score groups samples according to expected $\mathbf{X}$ in text prompt and evaluates end-to-end consistency in practical usage, while ``\textit{observe}'' score groups samples according to actually observed $\hat{\mathbf{X}}$ which is retrieved from videos and ignores condition generation errors. Notice that as text consistency improves, both scores should converge to the same. %$\sum_{\mathbf{S}}\sum_{i=1,\dots,|\mathbf{Y}_\mathbf{S}|}\operatorname{Var}(Y_i)/(|\mathbf{Y}_\mathbf{S}||\mathbf{S}|)$ as the score. 
%A variance close to 0 means the model reliably generates the same result under the same conditions, while a completely random model (50/50 split) reaches the theoretical maximum variance of 0.25.

%Since grouping is based on $\mathbf{X}$, errors arise if text consistency (level one) is imperfect. To address this, we use two scoring criteria: \textit{Groundtruth-based} grouping ($\mathbf{X}$), which evaluates end-to-end consistency, factoring in errors from incorrect condition generation; and \textit{observation-based} grouping ($\hat{\mathbf{X}}$), which measures consistency of the model’s actual condition-result mapping, ignoring condition generation errors and convenient to analyze the detailed model behavior.
%Notice as text consistency improves, both scores should converge to the same.
%Notice that our group is based on the value of $\mathbf{X}$, when level 1 is close to full score $1$, we expect $\mathbf{X} = \hat{\mathbf{X}}$. However, the current model is far from reaching this point, which will bring errors to our subsequent scoring. Therefore, we provide two different scoring criteria, that is, grouping $\mathbf{S}$ according to the groundtruth value described in text prompt ($\mathbf{X}$) or according to the observed value generated by the model ($\hat{\mathbf{X}}$). The former considers the end-to-end consistency performance in actual applications, and also includes some variance caused by incorrectly generating conditions; while the latter focuses on analyzing the functional consistency between the actual "condition-result" of the model, without considering the incorrect generation of conditions. It should be noted that as the text fidelity of the model gradually improves, these two scores should tend to converge to the same value.

% Let $d(V,\mathbf{S})$ measure the variance for samples in index set $\mathbf{S}$ on variable $V$. The metric $s_2^{\mathrm{truth}}\propto \sum_{\mathbf{S},V\in \mathbf{V}}d(V,\mathbf{S})$ calculates the variance of observed variables within each group, with lower variance indicating higher consistency. Similarly, we partition samples into groups $\mathbf{S}_{\mathbf{x}}$ based on observed root variables $\hat{\mathbf{X}}=\mathbf{x}$ and measure $s_2^{\mathrm{observe}}\propto \sum_{\mathbf{x},Y\in\mathbf{Y}}d(Y,\mathbf{S}_\mathbf{x})$. These metrics assess whether the model's internal rules produce stable and predictable outputs under consistent conditions, reflecting its ability to generalize from inputs to outputs.

\paragraph{Rule consistency}
The third level, our main and long-term goal, tests the model’s ability to learn and apply causal rules consistent with the real world. For one test case, we first calculate the accuracy for each rule (\ie for each outcome $Y_j\in\mathbf{Y}$).
For each outcome $Y_j=f(pa(Y_j))$, we sample prompts to make sure the groundtruth value of $Y_j$ is 50\% True and 50\% False. 
Having sampled videos $\mathbf{S}=\{s^{(1)},\dots,s^{(n)}\}$, the rule consistency is calculated as (1) the average accuracy $\sum_{i=1}^n \mathds{1}(Y^{(i)}_j=\hat{Y}^{(i)}_j)$, or (2) a threshold-based 0-1 score $\mathds{1}\{\operatorname{mean}[\mathds{1}(Y_j=\hat{Y_j})]\geq t\}$. 
Then the score of the test case take the average value among variables $\mathbf{Y}$. Here, we also distinguish two scores, ``\textit{truth}'' score using the groundtruth $pa(Y_j)$ and ``\textit{observe}'' score using the observed $\hat{pa}(Y_j)$ to get the expected $Y_j=f_j(pa(Y_j))$ where the latter isolates the direct cause-effect relationship, 
excluding errors from unexpected causes.

%For each outcome variable, we generate samples with balanced ground truth values (true or false) and measure accuracy using $s_3^{\mathrm{truth}}\propto \sum_{i,Y\in\mathbf{Y}}1(Y_i=\hat{Y}_i)$. Higher accuracy indicates that the model has learned consistent rules for inferring outcomes under varying conditions. 
%To mitigate text inconsistency, we also use observed root variables $\hat{\mathbf{X}}_i$ to compute $\tilde{Y}_i$ and measure $s_3^{\mathrm{observe}}\propto \sum_{i,Y\in\mathbf{Y}}1(\tilde{Y}_i=\hat{Y}_i)$. These metrics are the most critical, as they directly evaluate whether the model's learned rules align with the ground truth, reflecting its ability to capture and apply causal relationships.

\paragraph{Scores on samples} Though our experiments need comparison and evaluation on the scenario level where tens of videos could be involved, these metrics can be also applied to individual videos by redistributing the scores of each video according to its proportion in the overall score. It convenient to identify specific instances where the model's performance deviates, provide insights into its learning mechanisms or provide reward in a reinforcement learning stage. See Appendix~\ref{app:detailed_def_for_metrics} for detailed definitions and some example analysis in Appendix~\ref{app:example_score_based_analysis}.

% \section{An automatic generation of testbed}
% \subsection{The automatic generation of ground-truth causal systems}
% \subsection{Crowd experiments}
% \label{subsec:crowd_exp}

% \subsection{The automatic generation of test prompts}

% \subsection{Automatic testing}

\section{A benchmark of causal rule testing}


In this section, we use the 60 causal systems from 20 different scenarios (collected in our crowd experiments in Section~\ref{subsec:auto_label}) as a testbed to evaluate the causal learning of prevailing VGMs. We found that these models occasionally generate videos that are off-topic or with missing subjects and confusing logic. To avoid the score being affected too severely by the low-quality generation, we allowed the VLLM to answer ``N/A'' (in addition to yes/no) during answer retrieval, filtering out all observations marked as ``N/A'' across all metrics and reporting the ``N/A'' ratio in results. Table~\ref{tab:main_benchmark} shows our benchmarking results on some prevailing open- or closed-source models.
Here, rule consistency is calculated as the average accuracy score. For details on the tested models, testing costs, the impact of N/A, and sample efficiency, see Appendix~\ref{app:model_details} to \ref{app:sample_size_exp}.

%In crowd experiments in Section~\ref{subsec:auto_label} we have collected 60 causal systems with 20 different scenarios. We use them as a testbed for prevailing VGMs to test their causal learning ability. %The cost of benchmark can be found in \ref{app:cost}.
%We found that these models often generate videos that are far from the subject (such as blur, missing subjects, and confusing logic). For this reason, we additionally allow VLLM to answer N/A (besides yes/no) in the answer retrieval step, filtering all observations with N/A in all metrics. %We discuss about the N/A more in Appendix~\ref{app:affect_of_na}. 
%The rule consistency is calculated by the average accuracy score. About the details of the models, the cost of benchmarking, the affect of N/A, sample efficiency, and threshold-based rule consistency, see Appendix~\ref{app:model_details} to \ref{app:thre_score}.

%Table~\ref{tab:main_benchmark} shows our benchmarking results on some prevailing open or closed-source models. There are some important observation: %The results of threshold score are shown in Appendix~\ref{app:thre_score}.


\begin{table*}[htbp]
\centering

\caption{VACT benchmark on prevailing VGMs. The rule consistency is calculated by the ``average accuracy''.}

\label{tab:main_benchmark}
\begin{tabular}{lccccccc} 
\toprule
\multirow{2}{*}{\textbf{Model Names}} & \multirow{2}{*}{\textbf{N/A ratio}} & \multicolumn{2}{c}{\textbf{Text Consistency} $\uparrow$} & \multicolumn{2}{c}{\textbf{Generation Consistency} $\downarrow$} & \multicolumn{2}{c}{\textbf{Rule Consistency} $\uparrow$} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}  
& & all & root & truth & observe & truth & observe \\
 \midrule
% Random Generator& 1.0& -&- &- & -& -& - \\
% Stubborn Generator&0.0& 0.5& 0.5 & 0.0 & - &0.5 & -  \\
% Text-loyal Generator&0.0& 1.0 &1.0 &0.25 &0.25 & 0.5&0.5 \\
% Consistent Generator&0.0& 1.0 & 1.0 & 0.0 & 0.0 & $\sim$&$\sim$ \\
% Causal Perfect Generator&0.0& 1.0 & 1.0 & 0.0 & 0.0& 1.0& 1.0\\
 
% \midrule
CogVideoX1.5-5B & .07 & $.56\mathsmaller{\pm .01}$ & $.61\mathsmaller{\pm .01}$ & $.10\mathsmaller{\pm .00}$ & $.09\mathsmaller{\pm 
.01}$ & $.55\mathsmaller{\pm .01}$ & $.72\mathsmaller{\pm .02}$\\
CogVideoX-5B & .07 & $.58\mathsmaller{\pm .01}$ & $.64\mathsmaller{\pm .02}$ & $.09\mathsmaller{\pm .00}$ & $.09\mathsmaller{\pm .01}$ & $.56\mathsmaller{\pm .01}$ & $.71\mathsmaller{\pm .03}$ \\
CogVideoX-2B & .09 & $.56\mathsmaller{\pm .01}$ & $.63\mathsmaller{\pm .01}$ & $.09\mathsmaller{\pm .01}$ & $.09\mathsmaller{\pm .01}$ & $.59\mathsmaller{\pm .02}$ & $.72\mathsmaller{\pm .03}$ \\
VideoCrafter2  & .12 & $.55\mathsmaller{\pm .01}$ & $.58\mathsmaller{\pm .02}$ & $.08\mathsmaller{\pm .01}$ & $.06\mathsmaller{\pm .01}$ & $.53\mathsmaller{\pm .02}$ & $.73\mathsmaller{\pm .03}$ \\
Pyramid Flow & .10 & $.56\mathsmaller{\pm .01}$ & $.61\mathsmaller{\pm .02}$ & $.07\mathsmaller{\pm .00}$ & $.06\mathsmaller{\pm .01}$ & $.56\mathsmaller{\pm .01}$ & $.72\mathsmaller{\pm .03}$ \\
HunyuanVideo & .07 & $.58\mathsmaller{\pm .01}$ & $.63\mathsmaller{\pm .01}$ & $.08\mathsmaller{\pm .01}$ & $.07\mathsmaller{\pm .01}$ & $.57\mathsmaller{\pm .01}$ & $.70\mathsmaller{\pm .02}$ \\
\midrule
Pika & .10 & $.57\mathsmaller{\pm .01}$ & $.60\mathsmaller{\pm .01}$ & $.09\mathsmaller{\pm .00}$ & $.08\mathsmaller{\pm .01}$ & $.56\mathsmaller{\pm .01}$ & $.76\mathsmaller{\pm .02}$ \\
Hailuo & .07 & $.59\mathsmaller{\pm .01}$ & $.64\mathsmaller{\pm .01}$ & $.10\mathsmaller{\pm .00}$ & $.08\mathsmaller{\pm .01}$ & $.59\mathsmaller{\pm .01}$ & $.73\mathsmaller{\pm .02}$ \\
Gen-3 Alpha & .06 & $.63\mathsmaller{\pm .01}$ & $.63\mathsmaller{\pm .01}$ & $.08\mathsmaller{\pm .00}$ & $.08\mathsmaller{\pm .01}$ & $.57\mathsmaller{\pm .01}$ & $.74\mathsmaller{\pm .02}$ \\
Kling & .07 & $.63\mathsmaller{\pm .01}$ & $.64\mathsmaller{\pm .01}$ & $.07\mathsmaller{\pm .00}$ & $.07\mathsmaller{\pm .01}$ & $.57\mathsmaller{\pm .02}$ & $.71\mathsmaller{\pm .02}$ \\
\bottomrule
\end{tabular}

\end{table*}


In Table~\ref{tab:main_benchmark}, we observe that although certain closed-source models, such as Kling, demonstrated slightly better text consistency, and others, like Pika, showed marginally improved rule consistency, these differences were minor and not statistically significant. The fact that none of the existing models performed satisfactorily suggests that our benchmark can serve as a long-term objective for future research in this area. Given these observations, our main focus is to provide a comprehensive analysis and evaluation of the models. We explain the results as follows:

\paragraph{Text consistency}
The observed text accuracy ranged from 55\% to 65\%, only slightly above random guessing (50\%). This indicates that existing models \textbf{struggle to accurately generate variables from provided text}, regardless of whether causal or outcome variables are considered (with no significant difference between all and root cases). Although text fidelity has recently improved~\citep{sun2024soraseesurveytexttovideo}, our tests specifically require models to handle multiple variables simultaneously, including cases corresponding to less common scenarios. The low scores in our benchmarks highlight the models' difficulty in handling complex properties and uncommon situations. This implies that current models remain strongly \textit{limited to common scenarios} and \textit{lack the generalization capability} needed to effectively combine independent variables in more varied contexts, which is a necessary capacity for world simulators.

\paragraph{Generation consistency}
The generation consistency scores of all models are generally around 0.1. Consider that there is a random variable affecting the generation in each generation, we can use a two-point distribution to estimate the randomness. Because the variance of two-point distribution is $p(1-p)$, a value around 0.1 corresponds to approximately a 12\% deviation rate, meaning that 10 roughly 12\% of cases, model outputs vary significantly due to factors such as phrasing or random seed.

Overall, this indicates that models have learned relatively stable ``rule'', consistently producing similar outcomes for identical input variables $\mathbf{X}$.
However, this stability is not necessarily indicative of positive performance.
To better understand this, we consider text consistency and generation consistency results together. Although around 40\% of root variables being generated incorrectly (corresponding to around 60\% text consistency), the ``truth'' score and ``observation'' score in generation consistency remain closely aligned. This alignment occurs despite the fact that these scores categorize the same set of samples according to different criteria: the ground truth inputs $\mathbf{X}$ and the observed generated inputs $\hat{\mathbf{X}}$, respectively and there is a significant difference between these two values.

Such a pattern suggests that models may be \textbf{producing fixed outcomes} $\mathbf{Y}$ \textbf{regardless of variations in input variables} $\mathbf{X}$. This type of stability reflects what we call a ``\textit{degenerative}'' rule --- akin to a constant function. An illustrative example is shown in Figure~\ref{fig:bad_case}, where any object entering water invariably generates a splash. This behavior was further validated through manual inspection, as detailed in Appendix~\ref{app:analyze_gen_stable}.

\paragraph{Rule consistency} 
Finally, we directly evaluate the correctness of the rules learned by the models. The average ``truth'' rule accuracies are below 60\%, suggesting that the end-to-end rule accuracies are only slightly better than random guessing. Eliminating the influence of inaccurate conditions, the ``observe'' score shows that only around 70\% samples produces the same outcomes as in the real world. These findings indicate that poor performance in video generation consistent with real-world causal relationships is driven by both of these two main factors: models' misunderstanding of causal rules and their inability to accurately interpret and follow text instructions.

% Finally, we directly assess the correctness of the rules learned by the models. The average rule accuracies are below 60\% for the truth and only around 70\% for observation, with random guessing corresponding to 50\%. It suggests that both the misunderstanding of causal rules and the lacking to follow the correct text instruction leads to bad performance to generate videos obey the real-world causal relationships.

We calculate the threshold scores with threshold as $0.65$, $0.75$, $0.85$ and $0.95$. Here, we first calculate the average accuracy among samples for each causal rule and label it as $1$ if the average accuracy is larger than the threshold otherwise 0. The threshold score can reflect how many rules have been learned by VGMs with certain consistency. The results in Table~\ref{tab:metric_level_3_threshold} shows that only 14\%-26\% of the rules can match the groundtruth rules in 95\% of generation. This means that only a small number of causal relationships are learned by the model with a high degree of certainty.
And nearly 30\% of the rules have an accuracy below 65\%, which are almost unappreciated by the models. These findings clearly indicate that the models have not correctly understood the relationship between outcomes and causes (or parents), revealing weak rule learning of the current models.

\begin{table*}[htbp]
\centering
\caption{Metrics for rule consistency by applying threshold for each rule.}
\label{tab:metric_level_3_threshold}
\begin{tabular}{l *{8}{c}}  
\toprule
\textbf{Name} & 
\multicolumn{4}{c}{Truth} & 
\multicolumn{4}{c}{Observe} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-5} \cmidrule(lr){6-9}
\textbf{Threshold} & 0.65 & 0.75 & 0.85 & 0.95 & 0.65 & 0.75 & 0.85 & 0.95 \\
\midrule
CogVideoX1.5-5B  & $.19 \mathsmaller{\pm .04}$ & $.08 \mathsmaller{\pm .03}$ & $.02 \mathsmaller{\pm .01}$ & $.00 \mathsmaller{\pm .00}$ & $.61 \mathsmaller{\pm .05}$ & $.48 \mathsmaller{\pm .05}$ & $.30 \mathsmaller{\pm .05}$ & $.15 \mathsmaller{\pm .04}$ \\
CogVideoX-5B  & $.24 \mathsmaller{\pm .04}$ & $.10 \mathsmaller{\pm .03}$ & $.00 \mathsmaller{\pm .00}$ & $.00 \mathsmaller{\pm .00}$ & $.60 \mathsmaller{\pm .05}$ & $.45 \mathsmaller{\pm .05}$ & $.28 \mathsmaller{\pm .05}$ & $.14 \mathsmaller{\pm .04}$ \\
CogVideoX-2B  & $.32 \mathsmaller{\pm .05}$ & $.17 \mathsmaller{\pm .04}$ & $.06 \mathsmaller{\pm .02}$ & $.04 \mathsmaller{\pm .02}$ & $.59 \mathsmaller{\pm .05}$ & $.54 \mathsmaller{\pm .05}$ & $.34 \mathsmaller{\pm .05}$ & $.23 \mathsmaller{\pm .05}$ \\
VideoCrafter2 & $.18 \mathsmaller{\pm .04}$ & $.07 \mathsmaller{\pm .03}$ & $.01 \mathsmaller{\pm .02}$ 
& $.00 \mathsmaller{\pm .01}$ & $.59 \mathsmaller{\pm .05}$ & $.52 \mathsmaller{\pm .05}$ & $.36 \mathsmaller{\pm .05}$ & $.23 \mathsmaller{\pm .05}$ \\
Pyramid Flow   & $.23 \mathsmaller{\pm .04}$ & $.07 \mathsmaller{\pm .02}$ & $.00 \mathsmaller{\pm .00}$ & $.00 \mathsmaller{\pm .00}$ & $.63 \mathsmaller{\pm .04}$ & $.45 \mathsmaller{\pm .05}$ & $.32 \mathsmaller{\pm .05}$ & $.21 \mathsmaller{\pm .05}$ \\
HunyuanVideo  & $.30 \mathsmaller{\pm .05}$ & $.08 \mathsmaller{\pm .03}$ & $.03 \mathsmaller{\pm .02}$ & $.00 \mathsmaller{\pm .00}$ & $.56 \mathsmaller{\pm .04}$ & $.45 \mathsmaller{\pm .05}$ & $.30 \mathsmaller{\pm .05}$ & $.18 \mathsmaller{\pm .05}$ \\
\midrule
Pika  & $.27 \mathsmaller{\pm .05}$ & $.06 \mathsmaller{\pm .02}$ & $.00 \mathsmaller{\pm .00}$ & $.00 \mathsmaller{\pm .00}$ & $.66 \mathsmaller{\pm .05}$ & $.57 \mathsmaller{\pm .05}$ & $.35 \mathsmaller{\pm .05}$ & $.26 \mathsmaller{\pm .05}$ \\
Hailuo & $.28 \mathsmaller{\pm .05}$ & $.15 \mathsmaller{\pm .04}$ & $.05 \mathsmaller{\pm .02}$ & $.00 \mathsmaller{\pm .00}$ & $.66 \mathsmaller{\pm .05}$ & $.53 \mathsmaller{\pm .05}$ & $.35 \mathsmaller{\pm .06}$ & $.17 \mathsmaller{\pm .05}$ \\
Gen-3 Alpha  & $.26 \mathsmaller{\pm .05}$ & $.15 \mathsmaller{\pm .04}$ & $.03 \mathsmaller{\pm .02}$ & $.00 
\mathsmaller{\pm .00}$ & $.63 \mathsmaller{\pm .05}$ & $.51 \mathsmaller{\pm .05}$ & $.39 \mathsmaller{\pm .05}$ & $.23 \mathsmaller{\pm .05}$ \\
Kling  & $.23 \mathsmaller{\pm .04}$ & $.11 \mathsmaller{\pm .03}$ & $.05 \mathsmaller{\pm .02}$ & $.01 \mathsmaller{\pm .01}$ & $.60 \mathsmaller{\pm .04}$ & $.45 \mathsmaller{\pm .05}$ & $.29 \mathsmaller{\pm .06}$ & 
$.20 \mathsmaller{\pm .04}$ \\
\bottomrule
\end{tabular}
\end{table*}
\begin{table*}[htbp]
\centering

\caption{VACT benchmark on prevailing VGMs on human-sourced causal systems.}

\label{tab:human_benchmark}
\begin{tabular}{lc *{3}{cc}} 
\toprule
\multirow{2}{*}{\textbf{Model Names}} & \multirow{2}{*}{\textbf{N/A ratio}} & \multicolumn{2}{c}{\textbf{Text Consistency} $\uparrow$} & \multicolumn{2}{c}{\textbf{Generation Consistency} $\downarrow$} & \multicolumn{2}{c}{\textbf{Rule Consistency} $\uparrow$} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}  
& & all & root & truth & observe & truth & observe \\
 \midrule
CogVideoX1.5-5B & .11 & $.58\mathsmaller{\pm .01}$ & $.58\mathsmaller{\pm .02}$ & $.09\mathsmaller{\pm .01}$ & $.08\mathsmaller{\pm .01}$ & $.54\mathsmaller{\pm .02}$ & $.69\mathsmaller{\pm .02}$\\
\midrule
Pika & .18 & $.57\mathsmaller{\pm .01}$ & $.55\mathsmaller{\pm .02}$ & $.07\mathsmaller{\pm .01}$ & $.06\mathsmaller{\pm .01}$ & $.54\mathsmaller{\pm .02}$ & $.67\mathsmaller{\pm .02}$ \\
Hailuo & .14 & $.63\mathsmaller{\pm .01}$ & $.62\mathsmaller{\pm .02}$ & $.07\mathsmaller{\pm .01}$ & $.08\mathsmaller{\pm .01}$ & $.55\mathsmaller{\pm .01}$ & $.70\mathsmaller{\pm .02}$ \\
\bottomrule
\end{tabular}
\end{table*}


\paragraph{Human source evaluation}
We also benchmark some models using the 60 human-annotated causal systems (\ie the control group in crowd experiments) as an ablation study to support our automatic test case generation.
Except for the factors and rules in the test cases, other steps follow the same as the VACT system. The results are shown in Table~\ref{tab:human_benchmark}, where we conducted experiments using three video generation models: CogVideoX1.5-5B, Hailuo, and Pika. We obtain similar results. This serves an evidence for both the effectiveness of our automatic annotation and the validity of our benchmark conclusions. Other results like N/A ratio and threshold score are shown in Appendix~\ref{app:human-source}.

\section{Conclusion}


In this paper, we propose an automated system for modeling causal relationships in scenarios and evaluating the causal behavior of VGMs. By combining LLM's commonsense understanding with intervention experiments, our automatic system can assess the causal learning in VGMs across diverse domains, scenarios, and rules without any human annotation. We validated its effectiveness through crowd experiments and manual checks. We introduced three progressive causal metrics to comprehensively analyze the models' causal behavior. Using this system, we created a benchmark and identified key causal flaws in existing models. As a long-term target, this work lays the foundation for large-scale detection of shortcut or biased learning, supplementing comprehensive training datasets, or reinforcement learning.

\section{Limitation}
We acknowledge several limitations in our current work. First, although the LLMs can already generate high-quality testbeds, occasional errors may still occur. For scenarios requiring extremely high quality assurance, human check and assistance is still recommended. Second, our causal system construction involves certain simplifications, such as focusing only on visualized factors and binarizing variables, which may need refinement for more complex scenarios, such as extending binarization to multiple discrete levels. This remains our future work. Lastly, our evaluation assumes that model generate high-quality videos but some models still struggle with text understanding and coherent video generation, hindering the analysis of their causal behavior. We view our system as a forward-looking tool, believing that as video generation models rapidly improve, causal behavior analysis will become more critical.

% \section{Discussion}
% \textcolor{red}{move to appendix}
% \subsection{Sora's storyboard trick as a LLM-enhanced generation}
